A Logic of Reachable Patterns in Linked Data-Structures

We define a new decidable logic for expressing and checking invariants of programs that manipulate dynamically-allocated objects via pointers and destructive pointer updates. The main feature of this logic is the ability to limit the neighborhood of a node that is reachable via a regular expression from a designated node. The logic is closed under boolean operations (entailment, negation) and has a finite model property. The key technical result is the proof of decidability. We show how to express precondition, postconditions, and loop invariants for some interesting programs. It is also possible to express properties such as disjointness of data-structures, and low-level heap mutations. Moreover, our logic can express properties of arbitrary data-structures and of an arbitrary number of pointer fields. The latter provides a way to naturally specify postconditions that relate the fields on entry to a procedure to the fields on exit. Therefore, it is possible to use the logic to automatically prove partial correctness of programs performing low-level heap mutations.

==> properties.tex <==
\section{Finite Model Property for $\LRP$}\label{Sec:prop}

$\LRP$ formulas are preserved by an induced subgraph relation,
because $\LRP$ only allows existential formulas in pattern definitions.

\begin{Definition}\begin{Name}Induced Subgraph\end{Name}\label{def:substruct}
Let $S_1$ and $S_2$ be graphs over the same vocabulary $\voc$.
$S_1$ is an induced subgraph of $S_2$, denoted by $S_1 \sqsubseteq S_2$,
iff there is an \textbf{injective} function $h \colon S_1 \to S_2$ such that
\begin{enumerate}
\item for every constant symbol $\sigma \in \voc$, and for every $v\in S_1$,
$v$ is marked with $\sigma$ in $S_1$ if and only if  $h(v)$ is marked with $\sigma$ in $S_2$.
\item for every binary relation symbol $\sigma \in \voc$,
and every pair of nodes $v_1, v_2 \in S_1$,
there is an edge $(v_1,v_2)$ marked with $\sigma$ if and only if there is an edge $(h(v_1), h(v_2))$ in $S_2$
marked with $\sigma$.
\end{enumerate}
\end{Definition}
For a graph $S$, every subset $U$ of nodes of $S$ defines an induced subgraph of $S$,
which contains all edges that appear in $S$ between the nodes of $U$.

\begin{Lemma}\label{lem:substructPres}
Let $S_1$ be an induced subgraph of $S_2$ ($S_1 \sqsubseteq S_2$).
If $S_1 \models \posFormula{p_1}{R}{p_2}$ then $S_2 \models \posFormula{p_1}{R}{p_2}$.
Dually, if $S_2 \models \negFormula{p_1}{R}{p_2}$ then $S_1 \models \negFormula{p_1}{R}{p_2}$.
\end{Lemma}
Intuitively, if a graph $S$ satisfies formula $\psi = \posFormula{p_1}{R}{p_2}$,
then the result of adding new nodes to $S$ also satisfies $\psi$, because $\psi$ is existential.
However, the result of adding edges to $S$ need not satisfy $\psi$, because the patterns $p_1$ and $p_2$ in $\psi$
may contain negation of edges.

%\subsection{Finite Model Property}

$\LRP$ with arbitrary pattern definition formulas has a finite model property.
Even if formula $\phi$ has an infinite model, each subformula of $\phi$ that is satisfied by this model
has a finite witness. The union of these witnesses defines an induced subgraph of this model,
that also satisfies $\phi$, because $\LRP$ formulas are preserved by an induced subgraph relation.

\begin{Definition}\begin{Name}witness \end{Name}
\begin{itemize}
\item
A witness for a pattern $p(v_0) = \exists v_1, \ldots, v_k. \psi$ in a graph $S$ is a set of nodes in $S$
that constitute an assignment that satisfies $\psi$: $S_p, u_0, u_1, \ldots, u_k \models \psi(v_0, v_1, \ldots, v_k)$.
We say that the node $u_0$, assigned to $v_0$, is a ``central'' node of the witness.
\item
A witness for a regular expression $R$ in a graph $S$ is a path in $S$ labelled with a word $w$ in $R$.
If $w$ contains constant interrogations, $?c$ and $?\neg c$, then the corresponding nodes on the path are labelled with $c$
and $?\neg c$.
Note that the nodes and edges on a witness path for $R$ need not be distinct.
\item
A witness for a formula $\posFormula{p_1}{R}{p_2}$ in $\LRP$ is a graph $S$
that contains witnesses for $p_1$ and $p_2$, with ``central'' nodes $u_1$ and $u_2$,
respectively, and a witness path for $R$ from $u_1$ to $u_2$.
\end{itemize}
\end{Definition}
Note that a witness consists of a finite set of nodes, because
the regular expression requires a finite path and the patterns are existential formulas.
When a graph $S$ satisfies $\posFormula{p_1}{R}{p_2}$ (dually, $S$ violates  $\negFormula{p_1}{R}{p_2}$),
we say that $S$ has a witness for $\posFormula{p_1}{R}{p_2}$ (dually, a witness for $\negFormula{p_1}{R}{p_2}$).

\begin{SThe}{the:Finite}
\begin{Name}Finite Model Property\end{Name}
Every satisfiable $\LRP$  formula is satisfiable by a finite graph.
\begin{Sketch}
Consider an infinite graph $S$ that satisfies an $\LRP$ formula $\phi$.
We define a set of subformulas of $\phi$ that have witnesses in $S$:
\[
Q = \{ \negFormula{p_1}{R}{p_2} \mid \negFormula{p_1}{R}{p_2} \mbox{ appears in } \phi \mbox{ and } S \not \models \negFormula{p_1}{R}{p_2}\}
\]
Let $U$ be a subset of the nodes of $S$ that consists of
(i)~nodes of a witness of $\psi$, for every $\psi \in Q$, and
(ii)~all nodes of $S$ that are marked with the constants which appear in $\phi$.
Let $S'$ be an induced subgraph of $S$, defined by $U$.
$S'$ is finite, because each witness contains a finite set of nodes.

Let $\psi = \negFormula{p_1}{R}{p_2}$ be a subformula that appears in $\phi$.
If $S \models \psi$, then from \lemref{substructPres} we get that $S' \models \psi$,
because $S'$ is an induced subgraph of $S$, by construction.
If $S \not \models \psi$, then $\psi \in Q$, and by construction of $S'$, there is a witness in $S'$ for $\psi$, i.e., $S' \not \models \psi$.
Thus, $S' \models \phi$.
\end{Sketch}
\end{SThe}














%%%


==> response.tex <==
\section{Response}
\paragraph{COMPLEXITY}

This work was motivated by finding a balance between expressiveness,
decidability and complexity.

We proved decidability by reduction to MSO on trees (the reduction to MSO
preserves satisfiability but does not preserve equivalence). This allows us to
decide LBP2 formulas using MONA decision procedure.
We can show that the worst-case complexity of the satisfiability problem of
LBP2 is doubly-exponential, in contrast to MSO, which is non-elementary.
A doulbly-exponential decision procedure for LBP2 can directly construct a tree
automaton from a normal-form formula, and then check emptiness of the
automaton.

One exponential factor is a result of converting to normal form,
and another exponential factor arises from converting routing expressions to
deterministic automata. Experience in model checking indicates that this
complexity can be mitigated in many cases.
The worst-case complexity increases when "?c" constructs are used in complex
routing expressions. However, the verification conditions we generate do not
increase the complexity.


\paragraph{CONTRIBUTION}
This work is motivated by finding a balance between expressiveness,
decidability and complexity.

The practical importance of working with a theorem prover for computing
abstract transformers is shown by tools such as SLAM,BLAST,TVLA, and algorithms
reported in [VMCAI'04,TACAS'04,VMCAI'05].
Existing theorem provers cannot reason about reachability for data-structures
of arbitrary shapes, and may diverge.
In fact, several research groups are attempting to define a logic that handles
reachability and that is decidable, thus guarantees termination.

In [CAV'04] we tried to employ a decision procedure for MSO on trees to reason
about reachability.
This places a heavy burden on the specifyer to prove that the data-structures
in the program can be simulated using trees.
The current submission eliminated this burden by defining syntactic
restrictions on the formulas and showing a general reduction theorem.


The decidability result improves the state-of-the-art significantly.
In contrast to [CSL'04,VMCAI'05,MSR-TR-2005], LBP2 allows several binary
relations. This provides a natural way to
(i)specify invariants for data structures with multiple selectors (e.g., trees,
doubly-linked lists),
(ii)specify post-condition for procedures that mutate pointer fields of
data-structures, by expressing the relationships between fields before and
after the procedure (e.g., list reversal, which is beyond the scope of PALE),
(iii)easily generate verification conditions using a copy of the vocabulary for
each program location.


Review 1: We can provide a sketch of proof of Theorem 3.3 (VC are sound and
complete) for the final version.
Review 2: multiple selectors are used in Table 3 for specifying trees and
doubly-linked lists (more examples can be provided)


Review 3:
The decidable logic LBP2 is obtained from LBP by giving-up the ability to express certain shared graphs.
For example, we cannot write a formula whose set of models are only grids.
We observed that subtle changes to LBP2 break decidability, such as replacing
routing expression by general MSO formulas, as suggested by the referee.
The submission shows that LBP2 is expressible enough to write verification conditions of many programs.




\section{Conclusions}

In~\cite{CSL:eadtc}, we have found that defining decidable fragments of first-order logic with
transitive closure which are useful for program verification is a difficult task.
In this paper, we demonstrated that this is possible by combining the three principles:
(i)~allowing arbitrary boolean combinations of reachability constraints which are closed
(universal) formulas,
(ii)~defining reachability using regular expressions that denote
pointer access paths leading to patterns, and
(iii)~limiting the way patterns are formed.

The decidability result presented in this paper improves the state-of-the-art significantly.
In contrast to \cite{CSL:eadtc,BalabanPnueli:vmcai05,ShuvenduShaz:popl06}, $\LRP$ allows several binary
relations. This provides a natural way to
(i)specify invariants for data structures with multiple selectors (e.g., trees,
doubly-linked lists),
(ii)specify post-condition for procedures that mutate pointer fields of
data-structures, by expressing the relationships between fields before and
after the procedure (e.g., list reversal, which is beyond the scope of PALE),
(iii) generate verification conditions using a copy of the vocabulary for
each program location.

We are encouraged by the expressiveness of this simple logic and plan to explore its usage
for program verification and abstract interpretation.


==> soupy.tex <==
\section{Eliminating Positive Constants from Regular Expressions}


\begin{Lemma}\begin{Name}Elimination of $c$\end{Name}\label{lem:soupy}
Let $\voc$ be a vocabulary that does not contain $c$, and let $\voc'$ be $\voc \cup \{ c \}$.
For every regular expression $R$ over $\voc'$, there is a finite set of regular expressions
$D, \alpha_{i,j}, \beta_i, \gamma_i$ over $\voc$ (for $i=1,\ldots,m$ and $j=1,\ldots, m_i$),
such that for every graph $S$ over $\voc'$ and every pair of nodes $b,e \in S$,
\begin{center}
there is an $R$-path from $b$ to $e$ in $S$\\
if and only if \\
one of the following conditions holds:
\end{center}
\begin{enumerate}
\item there is a $D$-path from $b$ to $e$ in $S$, or
\item there is $i$, $1 \leq i \leq m$, such that
        \begin{enumerate}
        \item there is a $\beta_i$-path from $b$ to $c$ in $S$,
        \item for every $j = 1, \ldots, m_i$, there is a $\alpha_{i,j}$-path  from $c$ to $c$ in $S$,
        \item there is a $\gamma_i$-path from $c$ to $e$ in $S$.
       \end{enumerate}
\end{enumerate}
Moreover, the expressions $D, \alpha_{i,j}, \beta_i, \gamma_i$ can be computed from $R$.
\begin{Sketch}


\begin{Definition}\label{def:nequivStrings}\begin{Name}$n$-equivalence on strings\end{Name}
Strings $s_1$ and $s_2$ are $n$-equivalent ($s_1 \equiv_n s_2$)
if for every automaton $A$ with at most $n$ states, for every state $q, q' \in A$,
there is an $s_1$-path from $q$ to $q'$ in $A$ if and only if there is an $s_2$-path from $q$ to $q'$ in $A$.
\end{Definition}

\begin{Lemma}\label{lem:nequivStrings}
For every vocabulary $\Sigma$,
\begin{enumerate}
\item $\equiv_n$ is an equivalence relation,
\item $\equiv_n$ has finitely many equivalence classes,
\item for every equivalence class $C_i$, there is a \emph{characteristic regular expression} $\alpha_i$ such that
for every string $s \in \Sigma$,
$s \in C$ if and only if $s$ belongs to the language accepted by $\alpha_i$.
\end{enumerate}
\end{Lemma}


\begin{Lemma}\label{lem:combStrings}
Let $s_{1}, s_{2}, \ldots, s_{k}$, and $t_{1}, t_{2}, \ldots, t_{k}$ be strings over $\voc$.
If $s_{i} \equiv_n t_{i}$ for every $i = 1, \ldots, k$,
then $s_{1} (c) s_{2} (c) \ldots (c) s_{k} \equiv_n t_{1} (c) t_{2} (c) \ldots (c) t_{k}$.
\end{Lemma}

\begin{Lemma}\label{lem:characterizeString}
For every $n$, for every string $s$ over $\voc'$ that contains $c$, $s$ is $n-equivalent$.
\end{Lemma}


Now we are ready to prove \lemref{soupy}.
\paragraph{Input:} a regular expression $R$.
\paragraph{Task: } compute $D, \alpha_{i,j}, \beta_i, \gamma_i$ which satisfies the requirements of \lemref{soupy}.
%Given a regular expression $R$, the algorithm computes the set
%$D, \alpha_{i,j}, \beta_i, \gamma_i$ as follows:
\begin{enumerate}
\item Given regular expression $R$ over $\tau'$, construct an automaton $A$ that accepts $R$.
Let $n$ be the number of states in $A$.
Let $Q_n \eqdef \{ \alpha_1, \ldots, \alpha_n \}$ be the set of all
characteristic regular expressions for $\equiv_n$ over $\voc$.
\item A tuple $\beta, \gamma, \alpha_1, \ldots, \alpha_m \in Q_n$ is \textit{admissible for $R$}
if $R \cap \beta .( c.(\alpha_1 + \ldots + \alpha_m)  )^* . c . \gamma$ is not empty.
Find the set of all tuples admissible for $R$, $\beta_i, \alpha_{i,j}, \gamma_i$.
\item Let $D$ be $R \cap \voc^*$.
\end{enumerate}
\textbf{Correctness:}
Let $S$ be a graph over $\voc'$, and let $b, e$ be nodes in $S$.
Assume that there is an $R$-path from $b$ to $e$ in $S$, labelled with a string.
By definition of $R$, $s$ can be represented as $s_1 (c) s_2 (c) \ldots (c) s_k$,
and $s_i$ is over $\voc$.
Let $\beta$ be the characteristic expression for the $n$-equivalence class that contains $s_1$.
Let $\gamma$ be the characteristic expression for the $n$-equivalence class that contains $s_k$.
Let $\alpha_i$ be the characteristic expression for the $n$-equivalence class that contains $s_i$,
for $1 < i < k$.
Thus, $s$ is accepted by the regular expression $\beta . (c.(\alpha_1 + \ldots + \alpha_m))^* .\gamma$,
i.e., the tuple $\beta, \alpha_{i}, \gamma$ is admissible for $R$.
Therefore, requirements of  \lemref{soupy} hold for this tuple.

Assume that there is an admissible tuple $\beta, \alpha_1, \ldots, \alpha_m, \gamma$
and there is a $\beta$-path from $b$ to $c$ in $S$, denoted by $s_0$,
there is an $\alpha_i$-path  from $c$ to $c$ in $S$, denoted by $s_{i}$, for $i=1 , \ldots, m$,
and there is a $\gamma$-path from $c$ to $e$ in $S$, denoted by $s_{m+1}$.

From admissibility follows that there exists a string
$t \in R \cap \beta .( c.(\alpha_1 + \ldots + \alpha_m)  )^* . c . \gamma$,
which can be represented by $t_0 (c) t_1 (c) \ldots (c) t_{r}$.
Both $s_0$ and $t_0$ are in $\beta$, thus $s_0 \equiv_n t_0$, by \lemref{nequivStrings}(3).
Similarly, $s_{m+1} \equiv_n t_r$ because they are in $\gamma$.
Also, each $t_j$ satisfies $\alpha_{i_j}$, for some $i_j \in \{1, \ldots, m\}$.
Thus, $t_j \equiv_n s_{i_j}$.
Let $s$ be $s_0 s_{i_1}  s_{i_2} \ldots s_{i_{r-1}} s_{m+1}$.
By \lemref{combStrings}, $s \equiv_n t$, that is, $R$ cannot distinguish between $s$ and $t$.
Because $R$ accepts $t$, $R$ must accept $s$ as well.
That is, the path $s$ in $S$ is an $R$-path.
\end{Sketch}
\end{Lemma}



\begin{Lemma}\label{lem:soupyFormula}
Every $\LRPtwo$ formula is equivalent to an $\LRPtwo$ formula where $ c$ does not appear inside
any regular expression.
\begin{Sketch}
For every subformula $\posFormula{c_1}{R}{c_2}$ in $\LRP$ in which the regular expression $R$ contains $c$, transform $R$
into a finite set of regular expressions $\{ \beta_i, \alpha_{i,1}, \ldots, \alpha_{i,m_i}, \gamma_i \}_i \cup \{ D \}$
that do not contain $c$, according to \lemref{soupy}.
Replace $\posFormula{c_1}{R}{c_2}$ with
\[
\posFormula{c_1}{D}{c_2} \lor
\Lor_{i} \posFormula{c_1}{\beta_i}{c} \land
( \Land_{j=0, \ldots, m_i} \posFormula{c}{(\alpha_{i,j})^*}{c})
\land
\posFormula{c}{\gamma_i}{c_2}
\]
Similarly, for $R$ in every subformula $\negFormula{c_1}{R}{p_2}$ in $\phi$.
\end{Sketch}
\end{Lemma}

